An Extended View on Measuring Tor AS-level Adversaries

Tor provides anonymity to millions of users around the globe which has made it a valuable target for malicious actors. As a low-latency anonymity system, it is vulnerable to traffic correlation attacks from strong passive adversaries such as large autonomous systems (ASes). In preliminary work, we have developed a measurement approach utilizing the RIPE Atlas framework -- a network of more than 11,000 probes worldwide -- to infer the risk of deanonymization for IPv4 clients in Germany and the US. In this paper, we apply our methodology to additional scenarios providing a broader picture of the potential for deanonymization in the Tor network. In particular, we (a) repeat our earlier (2020) measurements in 2022 to observe changes over time, (b) adopt our approach for IPv6 to analyze the risk of deanonymization when using this next-generation Internet protocol, and (c) investigate the current situation in Russia, where censorship has been intensified after the beginning of Russia's full-scale invasion of Ukraine. According to our results, Tor provides user anonymity at consistent quality: While individual numbers vary in dependence of client and destination, we were able to identify ASes with the potential to conduct deanonymization attacks. For clients in Germany and the US, the overall picture, however, has not changed since 2020. In addition, the protocols (IPv4 vs. IPv6) do not significantly impact the risk of deanonymization. Russian users are able to securely evade censorship using Tor. Their general risk of deanonymization is, in fact, lower than in the other investigated countries. Beyond, the few ASes with the potential to successfully perform deanonymization are operated by Western companies, further reducing the risk for Russian users.

==> review.tex <==
\clearpage
\onecolumn

\fontfamily{sourcesanspro}\selectfont
\renewcommand{\quote}{\list{}{\rightmargin=\leftmargin\topsep=0pt}\item\relax}

\renewcommand\fix[1]{\textcolor{blue}{#1}}
\renewcommand\todo[1]{\textcolor{red}{#1}}

\fontfamily{lmr}\selectfont
\section*{Letter to the Reviewers}
\\~\\

\begin{large}
\noindent Dear reviewers,
\\~\\
thank you for you valuable feedback.\\
Following your suggestions, we carefully improved the paper. Among others, we included an additional section on limitations of our methodological approach and potential future research directions. 
Beyond, we proofread our paper again and corrected multiple editorial mistakes.\\
For a detailed response on the reviewers' comments, we refer to the remainder of this document. The changes in the paper are highlighted in red resp. blue color.
\\~\\
Sincerely,\\
Gabriel K. Gegenhuber on behalf of all authors
\end{large}

\vspace{0.5cm}
\subsection*{Reviewer \#2:}
\begin{quote}
In the abstract, you mention that you repeated the measurement from
2020. I would suggest that you add a year when it was repeated (2022).
Just so the reader is clear on when the repetition was done.
Otherwise, the paper is well written and structured.
\end{quote}
\fix{We added the missing date to clarify the time of our measurements.}

\begin{quote}
Extend the conclusion with possible limitations.
\end{quote}
\fix{We added a dedicated section (see Section~6) that discusses limitations and future research directions.}

\vspace{0.5cm}
\subsection*{Reviewer \#3:}
\begin{quote}
The authors present an empirical study on the anonymity of the Tor
network in the presence of AS-level adversaries. The article at hand is
based on a paper previously published by the authors, but contains
sufficient new material to warrant a publication.

Overall, the paper is well-written, with some minor issues (listed
below) that can be easily addressed. I appreciate the thoroughness of 
the empirical investigation as well as the timeliness of the study. The
methodology is sound (though I have a minor comment on that, see the
last comment below) and well explained. I recommend acceptance of the
paper.

Detailed comments:

* In the introduction, I would have appreciated a short explanation why
using BGP updates as a basis for the model is less reliable than the
approach at hand ([10] does have such an explanation). I do not doubt
that the measurement used here *is* actually better, it's just about the
explanation.
\end{quote}
\fix{We have extended the introduction explaining the advantage of tracerouting over BGP-based approaches. Briefly speaking, tracerouting reveals the actual paths that are taken by packets when traveling the Internet. We have additionally included a reference highlighting the fact that these BGP-based approaches overestimate Tor users' risk of deanonymization. We also included a brief explaination in Section~4 on methodology.
} 

\begin{quote}
* I notice an inconsistent use of tenses, in particular (but not only)
in Section 3 (switching between simple past, present perfect, and
present tense).
\end{quote}
\fix{We overworked Section 3 for consistency among tenses.}

\begin{quote}
* The first sentence in subsection 4.1 is incomplete.
\end{quote}
\fix{We added the missing reference to relays to the sentence.}

\begin{quote}
* Section 4.1 (page 4, right column, line 31): "Therefore, the
accumulated exit probabilities among top ASes became even more
centralized": became --> has become
\end{quote}
\fix{We corrected the use of past simple and changed it to present perfect.}

\begin{quote}
* Last sentence of Section 4.2 (page 5, right column, line 55): "and
exit relays did not change much" -> ... has not changed much
\end{quote}
\fix{We changed the tense from past simple to present perfect in the respective sections.}

\begin{quote}
* Page 7, line 14 (left column) should be : "as it does not host..."
\end{quote}
\fix{We corrected the sentence.}

\begin{quote}
* Page 8, line 51 (right column): "Second, AS2914 (NTTCOMMUNICATIONS-2)
was frequently observed for US based client ASes; nowadays, its
probability is...": first half seems to refer to 2020, but that is not
completely clear.
\end{quote}
\fix{We added the year 2020 to make it more clear to the reviewers.}

\begin{quote}
* Page 9, line 57 (left column): an -> and
* Page 9, line 58 (right column): its users -> their users
\end{quote}
\fix{We fixed the typos in respective locations.}

\begin{quote}
* Figure 9: Dashed lines should be explained.
\end{quote}
\fix{The dashed lines are contour lines highlighting points with 20\%,40\%,60\% and 80\% combined probability. We clarified this in the figure's caption as well as in the related section.}

\begin{quote}
* Page 12, line 38/39 (left column): Referring to 52.3\% as a moderate
probability appears strange; "Its" is not the correct word in the next
sentence.
\end{quote}
\fix{We adapted the wording and removed \textit{moderate} from the sentence.}

\begin{quote}
* Figures: Contrast and readability are not always optimal (light blue
and grey, in particular, might be hard to differentiate depending on the
device used for viewing).
\end{quote}
\fix{We removed the gray background on all images and replaced colors for some lines.
Further, we replaced the light gray data points on Figure 9 and 10 with black.}

\begin{quote}
* Overall: Could there be a bias due to the distribution of RIPE atlas
probes over ASes - in particular within Russia? (I have not really
thought this through, but this appears to be something that should be
discussed at least briefly).
\end{quote}
\fix{Thank you very much for this input. Section~6 briefly discusses the declining RIPE Atlas coverage in Russia, and its impact on the measurements.}

\vspace{0.5cm}
\subsection*{Reviewer \#4:}
\begin{quote}
Strong points:

-The critical analysis of a critical topic nowadays: anonymity
-Addition of current data
-Investigation of anonymity regarding Russia-Ukraine
-Comparison of IPV4 vs IPv6

Improvements:
-Review and improve figure 3 and 4 for black and white (grayscale)
printing
\end{quote}
\fix{
Figures 3 and 4 have been reworked. 
The light gray background has been changed to white, and colors with different saturation levels have been chosen for easier black and white readability.
We adjusted the light red to a darker red in Figure 4 to improve differentiation between red and green.
}

\begin{quote}
-Page 9 in line 57 "Russia and Germany" has a missing letter
\end{quote}
\fix{As also pointed out in the response to reviewer \#3, we added the missing letter.}

\begin{quote}
-Explain paths for future research in the topic
-Further discuss the limitations of the research presented
\end{quote}
\fix{We added a dedicated section (Section~6) that discusses limitations and future research directions.}

\vspace{0.5cm}
\subsection*{Reviewer \#6:}

\begin{quote}
Overall: This paper presents as an update on earlier work, but with a
couple of extra twists which make it sufficiently interesting for
publication.
As an update, the methods used have already been validated and there is
no real new insight.

I would however encourage the authors to look into the evolution of AS
ownership as something to monitor on a fairly regular basis to assess
how risks change through time.
\end{quote}
\fix{
Thank you for this remark.
We added context on the observed company/AS merges that occurred in the time period between our measurements, see Section~4.4.
Additionally, we added a related aspect on collaboration of ASes in Section~6, which could be an interesting topic for future work.
}



\begin{quote}
Note:
'We therefore advise to reconsider the placement of guard-, and exit
relays on the Internet. The former should be close to the clients, the
latter close to the destinations.'

This is not exactly new wisdom when it comes to using Tor.
\end{quote}
\fix{We rephrased the sentence to clarify that this is a problem known to the community. However, since this is still an existing challenge, we'd like to highlight it once more.}

\begin{quote}
Rephrase
- advertise up 700 Gbit/s of bandwidth

up to? upwards of? about? Not clear what is meant.
\end{quote}
\fix{We fixed the spelling to \textit{up to}.}

\begin{quote}
- investigating the status quo of IPv6 in the Tor network.

what status quo?
\end{quote}
\fix{We rephrased the sentence to be more precise.}

\begin{quote}
- consists of 6,559
relays?
\end{quote}
\fix{As also highlighted by reviewer \#3, this sentence was referring to \textit{relays}. We added the missing reference to the sentence.}

\begin{quote}
- we measure (1) 100%
at step (1) ?
\end{quote}
\fix{Yes, the sentence is referring to the forward and reverse paths shown in Figure 5. We added the reviewer's suggestion to make this more clear.}

\begin{quote}
- proneness to deanoymization attacks
deanonymization
\end{quote}
\fix{We are were sorry for this incosistencies. Together with the other occurrences, we corrected the spelling to \textit{deanonymization}.}

\begin{quote}
- as it does host a RIPE Atlas probe anymore.
does not
\end{quote}
\fix{Yes, as also mentioned by reviewer \#3, this AS \textit{does} not host a RIPE Atlas probe anymore.}

\begin{quote}
- in Germany and USA
and the
and you mix US and USA
\end{quote}
\fix{For consistency, we replaced all occurrences of USA with US.}

\begin{quote}
- In these ASes, we select RIPE Atlas probes and scheduled 1,194
traceroutes, as defined in Section 4.3;
we selected
\end{quote}
\fix{We changed the sentence accordingly to the reviewer's suggestion.}

\begin{quote}
- therefrom, 1,177 (98.6\%) were executed successfully (D1: 563/563, D2:
104/109, D3: 240/240, D4: 270/282).

out of which 1177
\end{quote}
\fix{We changed the sentence accordingly to the reviewer's suggestion.}

\begin{quote}
- an even higher chance of deanomyization
deanonymization
\end{quote}
\fix{We are very sorry for this inconsistencies. Together with the other occurrences, we corrected the spelling to \textit{deanonymization}.}

\begin{quote}
- 0.224 to deanoymize
you really have a random spelling problem will that word. I suggest you
do a systematic search on the 'deano' prefix across the paper.
\end{quote}
\fix{Together with the other occurrences, we corrected the spelling to \textit{deanonymization}.}

\begin{quote}
- tough with varying probabilities
though - or albeit
\end{quote}
\fix{We fixed the typo in the respective sentence.}

\begin{quote}
- in Russia an Germany.
and
\end{quote}
\fix{We fixed the typo in the respective sentence.}

\begin{quote}
- five new ASes with considerable chance to be along
with considerable chances of being
\end{quote}
\fix{We changed the sentence accordingly to the reviewer's suggestion.}

\begin{quote}
- to additional three use cases.
to three additional
\end{quote}
\fix{We changed the sentence accordingly to the reviewer's comment.}

\begin{quote}
Also

- ZWIEBELFREUNDE is truncated in table 4.
\end{quote}
\fix{That is correct, for enhanced readability, we changed it to ZWIEBELFR.}

\begin{quote}
- Every RIPE Atlas measurement is charged with credits, …

I am not sure why this is mentioned at that point (4.3). It looks more
like general discussions. 
\end{quote}
\fix{The authors agree with the reviewer and removed the part from section 4.3}.

